Online estimation of the inverse of the Hessian for stochastic optimization with application to universal stochastic Newton algorithms

This paper addresses second-order stochastic optimization for estimating the minimizer of a convex function written as an expectation. A direct recursive estimation technique for the inverse Hessian matrix using a Robbins-Monro procedure is introduced. This approach enables to drastically reduces computational complexity. Above all, it allows to develop universal stochastic Newton methods and investigate the asymptotic efficiency of the proposed approach. This work so expands the application scope of secondorder algorithms in stochastic optimization.

==> title.tex <==
\title{
Online estimation of the inverse of the Hessian for stochastic optimization with application to universal stochastic Newton algorithms}
\author{Antoine Godichon-Baggioni$^{(*)}$,
Wei Lu$^{(**)}$  and Bruno Portier$^{(**)}$\\
       $(*)$ Sorbonne Université, Laboratoire de Probabilités, Statistique et Modélisation  \\ 
       $(**)$ INSA Rouen Normandie, Laboratoire de Mathématiques de l'INSA \\     
         antoine.godichon$\_$baggioni@upmc.fr,  wei.lu@insa-rouen.fr,  bruno.portier@insa-rouen.fr \\
         \date{}
}
\editor{}
